Unsupervised clustering under the Union of Polyhedral Cones (UOPC) model

In this paper, we consider clustering data that is assumed to come from one of finitely many pointed convex polyhedral cones. This model is referred to as the Union of Polyhedral Cones (UOPC) model. Similar to the Union of Subspaces (UOS) model where each data from each subspace is generated from a (unknown) basis, in the UOPC model each data from each cone is assumed to be generated from a finite number of (unknown) \emph{extreme rays}.To cluster data under this model, we consider several algorithms - (a) Sparse Subspace Clustering by Non-negative constraints Lasso (NCL), (b) Least squares approximation (LSA), and (c) K-nearest neighbor (KNN) algorithm to arrive at affinity between data points. Spectral Clustering (SC) is then applied on the resulting affinity matrix to cluster data into different polyhedral cones. We show that on an average KNN outperforms both NCL and LSA and for this algorithm we provide the deterministic conditions for correct clustering. For an affinity measure between the cones it is shown that as long as the cones are not very coherent and as long as the density of data within each cone exceeds a threshold, KNN leads to accurate clustering. Finally, simulation results on real datasets (MNIST and YaleFace datasets) depict that the proposed algorithm works well on real data indicating the utility of the UOPC model and the proposed algorithm.

==> Algo.tex <==
\begin{algorithm}
   \caption{KNN-SC Algorithm}
  \begin{algorithmic}[1]
    \INPUT Noiseless Data: $X_1, X_2,..., X_N$, number of clusters $L$, threshold numbers $N_T$, scaling parameter $\tau$, gap parameter $\triangle \lambda$
    \OUTPUT Clustering Result $\zeta_1,\zeta_2,..., \zeta_K$
    \STATE Normalize each data by its $l_2$ norm such that $Y_i =\frac{X_i}{\|X_i\|_{l_2}}$
    \STATE \text{For each data $Y_{i:i=1,...,N}$, calculate the pairwise distance} $dist(Y_i, Y_{j:j\neq i}) = \|Y_i -Y_j\|_{l_2}$ and generate the sorted the index array  $I_i$ that is ordered by the distance from small to large
	\FOR{$k \in \{2,3,..,N_T \}$}
	\STATE Build affinity matrix $A_k$: $A_k(i,I_i(1:k)) = e^{-dist(Y_i, Y_{I_i(1:k)})/\tau} $ 
	\STATE Define $D_k$ to be diagonal matrix whose (i,i)-element is the sum of $A_k$'s i-th row and construct the Laplacian Matrix $L_k = D_k^{-1/2}A_kD_k^{-1/2}$
	\STATE Calculate the eigenvalue of $L_k$, sort the eigenvalue from large to small and count the the number of eigenvalues $C_k$ until the difference between the adjacent eigenvalue changes more than $\triangle \lambda$
	\ENDFOR
	\STATE If there exists a set of k such that $C_k$ equals K, then let the optimal number of neighbors $K^*$ be the median the set; If there is no such k that satisfying $C_k$ equals K, then let $K^*$ as the smallest of k such that $C_k < K$
	\STATE Apply Spectral Clustering corresponds to $A_{K^*}$ and return the clustering result $\zeta_1,..., \zeta_K$
  \end{algorithmic}
\end{algorithm}
